Polynomial 2D Biharmonic Coordinates for High-order Cages

We derive closed-form expressions of biharmonic coordinates for 2D high-order cages, enabling the transformation of the input polynomial curves into polynomial curves of any order. Central to our derivation is the use of the high-order boundary element method. We demonstrate the practicality and effectiveness of our method on various 2D deformations. In practice, users can easily manipulate the Bezier control points to perform the desired intuitive deformation, as the biharmonic coordinates provide an enriched deformation space and encourage the alignment between the boundary cage and its interior geometry.

==> src/fig-only.tex <==


%\paragraph{More examples}

\begin{figure*}[t]
  \centering
  \begin{overpic}[width=0.99\linewidth]{more_compare_mvc}
    {
\put(7,-1.5){\small Rest pose}
 \put(28,-1.5){\small Cubic MVC}
 \put(55,-1.5){\small Poly GC}
 \put(84,-1.5){\small Ours}
    }
  \end{overpic}
  \vspace{-0mm}
  \caption{
  Comparisons with Cubic MVC and PolyGC on two examples using the same polygonal cages. At the bottom, we use weighted coordinates with $w=0.5$.
  }
  \label{fig:more-cmp}
\end{figure*}

\begin{figure*}[t]
  \centering
  \begin{overpic}[width=1.0\linewidth]{compare_our_octopus}
    {
 \put(10,-1.5){\small Rest pose}
 \put(28,-1.5){\small $w=0$ (CurvedGC)}
 \put(57,-1.5){\small $w=0.5$}
 \put(84,-1.5){\small $w=1$}
    }
  \end{overpic}
  %\vspace{-2mm}
  \caption{
   Comparisons with CurvedGC on two examples using the same cubic cages.
  }
  \label{fig:more-curvedcmp}
\end{figure*}

==> src/newmethod.tex <==
\section{method}\label{sec:method}
We provide a systematic review of the entire process for deriving the biharmonic coordinates in Section~\ref{sec:revisit}, then introduce our closed-form coordinates for high-order cages based on high-order BEM in Section~\ref{sec:HighOrderBEM}, and finally discuss the deformation controls in Section~\ref{sec:deformation}.

\subsection{Revisiting Biharmonic Coordinates}\label{sec:revisit}
Biharmonic coordinates are derived as the solution to the biharmonic Dirichlet problem (refer to Equation 4 in \cite{Weber2012}), obtained using the boundary element method (BEM).

\begin{equation}\label{equ:bihPDE}
\begin{aligned}
    &\Delta^2 f(\eta) = 0, \quad \eta \in \Omega, \\
    &f(\xi) = g_1(\xi), \quad \xi \in \partial \Omega, \\
    &\frac{\partial f}{\partial n}(\xi) = g_2(\xi), \quad \xi \in \partial \Omega.
\end{aligned}
\end{equation}


\paragraph{boundary element method}
In the boundary element method, the differential equation within the region is first converted into an integral equation on the boundary. The boundary is then discretized into finite-sized boundary elements, and the boundary integral equation is transformed into an algebraic equation. This effectively converts the problem of solving the partial differential equation into the problem of solving an algebraic equation for the unknown nodal values.

\paragraph{boundary integral equations}
Using Green's theorem and the fundamental solution, the differential equation~\eqref{equ:bihPDE} is transformed into the following boundary integral equations:
\begin{equation}\label{equ:BIE1}
\begin{aligned}
f(\eta) &=
\int\limits_{\xi \in \partial \Omega}
f(\xi) \frac{\partial G_1}{\partial n}(\xi, \eta)d\xi -
\int\limits_{\xi \in \partial \Omega}
G_1(\xi, \eta) \frac{\partial f(\xi)}{\partial n}d\xi \\
+ &\int\limits_{\xi \in \partial \Omega}
\Delta f(\xi) \frac{\partial G_2}{\partial n}(\xi, \eta)d\xi -
\int\limits_{\xi \in \partial \Omega}
G_2(\xi, \eta) \frac{\partial \Delta f(\xi)}{\partial n}d\xi,
\end{aligned}
\end{equation}

\begin{equation}\label{equ:BIE2}
\begin{aligned}
\Delta f(\eta) =
\int\limits_{\xi \in \partial \Omega}
\Delta f(\xi) \frac{\partial G_1}{\partial n}(\xi, \eta)d\xi -
\int\limits_{\xi \in \partial \Omega}
G_1(\xi, \eta) \frac{\partial \Delta f(\xi)}{\partial n}d\xi,
\end{aligned}
\end{equation}
where $G_1$ and $G_2$ are the fundamental solutions of the 2D harmonic and biharmonic equation, respectively. Specifically, these are given by $G_1(\xi,\eta)=-\frac{1}{2 \pi}\ln\|\xi-\eta\|$ and $G_2(\xi,\eta)=-\frac{\|\xi-\eta\|^2}{8 \pi}(\ln\|\xi-\eta\|-1).$
In the integral equations, since \( f \) and \( \partial f/\partial n \) are given in~\eqref{equ:bihPDE}, the unknown functions only contain \( \Delta f \) and \( \partial \Delta f/\partial n \). Once we have solved for all the unknown function values of \( \Delta f \) and \( \Delta f/\partial n \) on the boundary, substituting them into~\eqref{equ:BIE1} yields the value of $f$ at any point within the domain $\Omega$, which is the solution to~\eqref{equ:bihPDE}.
%
%Although \eqref{equ:BIE1} and \eqref{equ:BIE2} are valid for any point \(\eta\) within the domain, to solve for \(\Delta f\) and \(\partial \Delta f/\partial n\) on the boundary, \(\eta\) must be moved to the boundary (denoted as \(\eta'\)). 
To solve for \(\Delta f\) and \(\partial \Delta f/\partial n\) on the boundary, \(\eta\) must be moved to the boundary (denoted as \(\eta'\)) in \eqref{equ:BIE1} and \eqref{equ:BIE2}. 
%
At this point, the integrals involved become singular, but the limits of the integrals still exist.

\paragraph{Discretization and Solution}
In general, solving integral equations numerically involves two main steps: discretization and solving the resulting system of algebraic equations. 

The discretization process consists of two sub-steps. First, the boundary is divided into finite-sized boundary elements. Second, the functions defined on the boundary are approximated within each element using interpolation. 
In the biharmonic coordinates for 2D polygonal cages \cite{Weber2012} and 3D triangular cages \cite{thiery2024biharmonic}, the boundary is piecewise linear and is naturally discretized into piecewise linear elements. Within each element, \(f\) and \( \partial f/\partial n\) are represented using piecewise linear and piecewise constant functions, respectively. The unknowns \(\Delta f\) and \(\Delta f/\partial n\) are approximated using piecewise linear and piecewise constant functions as well. 
By representing the functions in terms of their values at the nodes of the boundary elements, an algebraic system of equations is established based on the evaluation of \(\eta'\) at different boundary points.

To solve the system of algebraic equations, \cite{Weber2012} substitute the algebraic constraints generated by~\eqref{equ:BIE2} into the equations derived from~\eqref{equ:BIE1}. In 3D, \cite{thiery2024biharmonic} proposed simultaneously minimizing the two constraints, which resulted in better-behaved deformation outcomes.
%At this point, we approximate \( \Delta f \) and \( \partial \Delta f/\partial n \) by searching for \( g \) and \( g_n \) within the space of piecewise linear functions and the space of piecewise constant functions, respectively, on the boundary. 



\begin{figure}[t]
  \centering
  \begin{overpic}[width=1.0\linewidth]{blank}
    {
 \put(83,-3.5){\small Ours}
    }
  \end{overpic}
  %\vspace{-2mm}
  \caption{
  A schematic diagram for explaining the problem?
  }
  \label{fig:schematic}
\end{figure}

\subsection{Higher-order boundary element method}\label{sec:HighOrderBEM}
Compared to the previously mentioned linear boundary element method, the high-order boundary element method has been proven to offer higher accuracy and faster solution speed for solving many types of equations~\cite{gravenkamp2019high}.

When solving for biharmonic coordinates, the high-order boundary element method offers additional advantages: it enables deformations from straight edges to curved edges and deformations from curved edges to curved edges. The main idea is that when we use linear elements combined with high-order basis functions to represent the functions \( g_1 \), \( g_2 \), \( \Delta f \), and \( \Delta f/\partial n \), the deformation from straight edges to curved edges is permitted. Furthermore, when high-order elements are employed, the deformation from curved edges to curved edges becomes possible.
More generally, we will next focus on describing how to achieve deformations from curved edges to curved edges, based on the high-order boundary element method.

% \paragraph{Straight segment to polynomial curves}
% Generally, we present here how to solve the partial differential equation in (1), where \(\Omega\) has curved boundaries, and 
% $f$ is a smooth function. Let the boundary curve \(\partial \Omega\) be divided into \(m\) non-overlapping small curve segments $\Omega_i$. In this case, traditional linear elements and linear functions are no longer a good approximation for the boundary.  Instead, we can adopt high-order boundary element methods that employ higher-order elements and shape functions. The higher-order boundary finite element method has been proven to provide greater accuracy and efficiency in solving many differential equations~\cite{gravenkamp2019high}.

\paragraph{Higher-order Discretization}
High-order boundary element methods employ higher-order elements and shape functions.
We primarily focus on a single boundary element, parametrized as \( c_j(t): [0, 1] \to \mathbb{R}^2 \).
For an \(l\)-th order element, \(c_j\) is an \(l\)-th degree polynomial, representing a single edge of the initial cage as an \(l\)-th order \Bezier curve.

In this case, we typically assume that \(g_1\) is an \(n\)-th degree polynomial function on the element:
\begin{equation}\label{equ:g}
\begin{aligned}
    g_1(t)=\sum_{i=0}^n g_{1,i}B_i^n(t), g_2(t)=s\frac{\|g_1'(t)\|}{\|c'(t)\|}.
    \end{aligned}
\end{equation}
The selection of \(g_2\) is inspired by polynomial Green coordinates~\cite{MichelThiery2023}, where $s$ is a scaling factor.
Here, \( B_i^n \) represents the Bernstein basis functions, which we use to achieve a more direct deformation method. 
$g_1(t)$ implies that the deformed edge of the cage is an \(n\)-th degree polynomial curve. To ensure deformation continuity, we choose \(n \geq l\).

Furthermore, we approximate \(\Delta f\) using a \(k\)-th order polynomial and \(\Delta f/\partial n\) using a \((k-1)\)-th order polynomial:
\begin{equation}\label{equ:Df}
\begin{aligned}
    \Delta f(t)=\sum_{i=0}^k h_{1,i}B_i^k(t), \Delta f/\partial n(t)=\sum_{i=0}^{k-1} h_{2,i}B_i^{k-1}(t),
    \end{aligned}
\end{equation}
We choose \(k \geq n\) to ensure the ability to reproduce affine transformations.

Substituting \eqref{equ:g} and \eqref{equ:Df} into \eqref{equ:BIE1} and \eqref{equ:BIE2} yields the discretized boundary integral equations.
{\small
\begin{equation}
	\begin{aligned}
		f(\eta) &= \sum_{j=1}^{m} \int_{0}^1 \frac{\partial G_1(c_j(t),\eta)}{\partial n} g_1(t) \, dt 
		- \sum_{j=1}^{m} \int_{0}^1 g_2(t) G_1(c_j(t),\eta) \, dt\\
		&+ \sum_{j=1}^{m} \int_{0}^1 \frac{\partial G_{2}(c_j(t),\eta)}{\partial n} \Delta f(t) \, dt 
		- \sum_{j=1}^{m} \int_{0}^1 \frac{\partial \Delta f(t)}{\partial n} G_{2}(c_j(t),\eta) \, dt\\
	\end{aligned}
\end{equation}
\begin{equation}
	\begin{aligned}
		\Delta f(\eta)
		= \int\limits_{t=0}^1 \frac{\partial G_1(c_j(t),\eta)}{\partial n} \Delta f(t) \, dt  
        + \int\limits_{t=0}^1 \frac{\partial \Delta f(t)}{\partial n} G_1(c_j(t),\eta) \, dt 
	\end{aligned}
\end{equation}
}

Evaluating the integrals leads to:
\begin{equation}\label{equ:dis_Int1}
    f(\eta) = \sum_{j=1}^m \left(\sum_{i =0}^n \phi_{ij}(\eta) g_{1,i} +  \psi_j(\eta) g_{1,i}^{\perp} 
+ \sum_{i \in V} \tilde{\phi}_i(\eta) h_{1,i} +  \tilde{\psi}_j(\eta) h_{2,i}\right),
\end{equation}
\begin{equation}\label{equ:dis_Int2}
   \Delta f(\eta) = \sum_{j=1}^m \left(\sum_{i \in V} \tilde{\phi}_i(\eta) h_{1,i} + \sum_{j \in T} \tilde{\psi}_j(\eta) h_{2,i}\right),
\end{equation}
If \(\eta\) lies strictly within the interior of \(\Omega\), the theorem 1 in \cite{liu2024polygc} provides the method for computing these integrals.
\paragraph{Polynomial Biharmonic Coordinates}
To obtain the system of algebraic equations, we sample \(\eta\) on the boundary. In this case, singular integrals need to be computed. However, the theorem in \cite{liu2024polygc} is no longer applicable as it becomes unstable for calculations near the boundary. We performed additional computations for this case; see the supplementary materials for details.

Substituting \(\eta\) on the boundary into \eqref{equ:dis_Int1} and \eqref{equ:dis_Int2} yields the following matrix constraints:
\begin{equation}
    (\Phi_L - M_L)L' + \Psi_L D' = 0,
\end{equation}

\begin{equation}
    (\Phi_V - M_V)V' + \Psi_V N' + \bar{\Phi}_V L' + \bar{\Psi}_V D' = 0.
\end{equation}

Two methods were used to solve the system of algebraic equations: one strictly enforces the Dirichlet boundary conditions, while the other applies them more leniently. They lead to the following expression for our regularized biharmonic coordinates:
\begin{equation}
    \begin{aligned}
\mathcal{M}' &= \big[ \Phi_M + (\dot{\Phi}_M C_L + \ddot{\Psi}_M C_D)(M_V - \Phi_V) \big] V' \\
&\quad + \big[ \Psi_M - (\dot{\Phi}_M C_L + \ddot{\Psi}_M C_D)\Psi_V \big] N'  \\
&= \big[ \Phi_M + \dot{\Phi}_M C_{11} + \ddot{\Psi}_M C_{12} \big] V'  \\
&\quad + \big[ \Psi_M + \dot{\Phi}_M C_{21} + \ddot{\Psi}_M C_{22} \big] N'  
\end{aligned}
\end{equation}
To improve the accuracy of numerical solutions, three methods can be employed:  1. Increase the number of boundary elements to expand the discretized approximation space. When the number of boundary elements is sufficiently large, we nearly obtain all the values of \( df \) and \( df_n \) on the boundary, and the resulting \( f \) almost satisfies all the boundary conditions. However, increasing the number of boundary elements leads to a larger, denser matrix for solution.  
2. Increasing the degree of \(k\), similar to Method 1, results in a larger approximation space with greater degrees of freedom. In our experiments, we found that Methods 1 and 2 yield comparable results.
3. Increase the number of sampling points \( \eta' \). This results in an over-constrained system of equations, which enforces the integral equations to hold at more points in the least-squares sense, thereby making the deformation results appear smoother.


\subsection{Variational Neumann condition}\label{sec:deformation}
In \eqref{equ:g}, different choices of \( s \) correspond to different Neumann boundary conditions. We now provide several methods for
automatically deducing boundary derivatives from boundary positions alone. Which method to choose depends on
the effect that the user wants to achieve, thus application-dependent.
\paragraph{unit} We set $s_j=1$. The deformation will tend to preserve angles between any two intersecting curves in the vicinity of the boundary with the added value of interpolating the boundary (with possibly more shear in the interior).

\begin{figure}[t]
  \centering
  \begin{overpic}[width=1.0\linewidth]{blank}
    {
 \put(83,-3.5){\small Ours}
    }
  \end{overpic}
  %\vspace{-2mm}
  \caption{
  various methods for solving the linear equation.
  }
  \label{fig:linear-solving}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{overpic}[width=1.0\linewidth]{scale}
    {
    \put(33,-3.5){\small unit}
    \put(60,-3.5){\small AHAP}
 \put(83,-3.5){\small AAAP}
    }
  \end{overpic}
  %\vspace{-2mm}
  \caption{
  with or without scaling.
  }
  \label{fig:scaling}
\end{figure}

\paragraph{As-harmonic-as-possible}
In more complicated scenarios, when the source and target cages are significantly different, a more sophisticated way to choose $s_j$ is required. Since we consider harmonic coordinates to be the preferred choice for deformation among all real coordinate recipes, the closest to this is what we call the As-Harmonic-As-Possible (AHAP) map that still satisfies the user constraints.

We define the harmonicity of a \textit{biharmonic} function $f(x)$ as
\begin{equation}
E_{\text{AHAP}}(f) = \int_{\partial \Omega} \|\Delta f(x)\|^2 ds, 
\end{equation}
where the integration is done solely on the boundary. Recall that $\Delta f(x)$ is harmonic, hence achieves minimum/maximum values on the boundary. Therefore minimizing $\|\Delta f(x)\|^2$ on the boundary bounds its values in the interior. We also experimented with integrating over the entire domain and obtained similar results. In our discrete setting, (20) becomes $\|l\|^2$ where $l = Bf + Cd$ and $d_j = s_j \hat{n}_j$. Thus, given the vector of boundary values $f$, the only unknowns are the scalars $s_j$.


\paragraph{As-affine-as possible}

\begin{equation}
E_{\text{AAAP}}(f) = \int_{\partial \Omega} \| f'(x)\|^2 ds, 
\end{equation}
